Script-Strategy Aligned Generation: Aligning LLMs with Expert-Crafted Dialogue Scripts and Therapeutic Strategies for Psychotherapy

Chatbots or conversational agents (CAs) are increasingly used to improve access to digital psychotherapy. Many current systems rely on rigid, rule-based designs, heavily dependent on expert-crafted dialogue scripts for guiding therapeutic conversations. Although advances in large language models (LLMs) offer potential for more flexible interactions, their lack of controllability and explanability poses challenges in high-stakes contexts like psychotherapy. To address this, we conducted two studies in this work to explore how aligning LLMs with expert-crafted scripts can enhance psychotherapeutic chatbot performance. In Study 1 (N=43), an online experiment with a within-subjects design, we compared rule-based, pure LLM, and LLMs aligned with expert-crafted scripts via fine-tuning and prompting. Results showed that aligned LLMs significantly outperformed the other types of chatbots in empathy, dialogue relevance, and adherence to therapeutic principles. Building on findings, we proposed ``Script-Strategy Aligned Generation (SSAG)'', a more flexible alignment approach that reduces reliance on fully scripted content while maintaining LLMs' therapeutic adherence and controllability. In a 10-day field Study 2 (N=21), SSAG achieved comparable therapeutic effectiveness to full-scripted LLMs while requiring less than 40\% of expert-crafted dialogue content. Beyond these results, this work advances LLM applications in psychotherapy by providing a controllable and scalable solution, reducing reliance on expert effort. By enabling domain experts to align LLMs through high-level strategies rather than full scripts, SSAG supports more efficient co-development and expands access to a broader context of psychotherapy.

==> package.tex <==
% Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% Standard package includes
\usepackage{times}
\usepackage{latexsym}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

% If the title and author information does not fit in the area allocated, uncomment the following
%
%\setlength\titlebox{<dim>}
%
% and set <dim> to something 5cm or larger.

% =========================================================================================

\usepackage{acronym}
\usepackage{enumitem} % Add this line

\usepackage{subfigure} 
\usepackage{subcaption}  

==> tables/dataset_statistics.tex <==
% \newcommand{\datasetsmall}{\fontsize{7.9pt}{9.8pt}\selectfont}

\begin{table}[!h]
\centering
% \datasetsmall
\footnotesize
\renewcommand{\arraystretch}{1.10}
\setlength{\tabcolsep}{8.0pt} % Reduce column separation
% \begin{tabular}{\textwidth}{@{\extracolsep{\fill}}p{3.1cm}p{3.4cm}p{3cm}@{}}
\begin{tabular}{lrr}
\hline
\textbf{Dataset} & \textbf{Intervention} & \textbf{Diagnosis} \\ \hline
Psychotherapeutic Topics & 26 & 43 \\ 
% \hline
Turns (Per Topic) & 53 & 15 \\ 
Utterances (Total) & 1400 & 680 \\ \hline 
% Dialogue Turns  &  & 0 \\ \hline
\end{tabular}
\vspace{-0mm}
% \caption{Statistics of the dataset with expert-defined dialogues for intervention (using MI and CBT) and mental diagnosis (using DSM-5).}
\caption{Statistics of the dataset with expert-crafted dialogue scripts for intervention and mental diagnosis.}
\label{tab:dataset_statistics}
\vspace{-0mm}
\end{table}

==> tables/descriptive_two_scenarios.tex <==
\begin{table*}[!htbp]
\centering
\renewcommand{\arraystretch}{0.960}
\footnotesize
\setlength{\tabcolsep}{2pt} % Reduce column separation
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{1.5cm}p{3.2cm}p{1.7cm}p{2.5cm}@{}}
\hline
\multirow{2}{*}{\textbf{Measures}} & \multirow{2}{*}{\textbf{Conditions}} & \multicolumn{2}{c}{\textbf{Scenarios}} \\ \cline{3-4}
 &  & \textbf{Behavioral Intervention} & \textbf{Mental Diagnosis} \\ \hline

\multirow{4}{*}{Pre-survey} 
 & Frequence of usage & 3.14 & 0 \\ \cline{2-4} 
 & Experience with chatbot & 3.23 & 0 \\ \cline{2-4} 
 & Familiarity of chatbot & 3.44 & 0 \\ \cline{2-4} 
 & Attitude toward chatbot & 3.40 & 0 \\ 
\hline

\multirow{4}{*}{Linguistic Quality} 
 & Rule-based chatbot & 3.66 & 0 \\ \cline{2-4} 
 & Pure LLM chatbot & 3.76 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.60 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.95 & 0 \\ 
\hline

\multirow{4}{*}{Usability} 
 & Rule-based chatbot & 3.60 & 0 \\ \cline{2-4} 
 & Pure LLM chatbot & 3.56 & 0  \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.61 & 0\\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.82 & 0 \\ 
\hline

\multirow{4}{*}{Dialogue Relevance} 
 & Rule-based chatbot & 3.26 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 3.09 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.38 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.39 & 0 \\ 
\hline

\multirow{4}{*}{Empathy} 
 & Rule-based chatbot & 2.53 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 2.99 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 2.94 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.07 & 0 \\ 
\hline

\multirow{4}{*}{Engagement} 
 & Rule-based chatbot & 2.58 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 2.72 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 2.58 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 2.90 & 0 \\ 
\hline

\multirow{4}{*}{Perceived MI} 
 & Rule-based chatbot & 3.13 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 3.13 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.31 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.74 & 0 \\ 
\hline

\multirow{4}{*}{Therapeutic Alliance} 
 & Rule-based chatbot & 3.31 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 3.33 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.33 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.58 & 0 \\ 
\hline

\multirow{4}{*}{Motivation} 
 & Rule-based chatbot & 2.86 & 0\\ \cline{2-4} 
 & Pure LLM chatbot & 3.00 & 0 \\ \cline{2-4} 
 & LLM chatbot (FT) & 3.00 & 0 \\ \cline{2-4} 
 & LLM chatbot (Prompted) & 3.42 & 0 \\ 
\hline
\end{tabular*}
\caption{Descriptive statistics of the results.}
\label{tab:descriptive}
\vspace{-6mm}
\end{table*}

==> tables/dialogue_overview.tex <==
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.0}
\small
\setlength{\tabcolsep}{20.0pt} % Reduce column separation
% \begin{tabular}{\textwidth}{@{\extracolsep{\fill}}p{3.0cm}p{4.2cm}p{1.9cm}p{1.9cm}@{}}
\begin{tabular}{lcccc}
\hline
\multirow{1}{*}{Therapeutic Question} & \multirow{1}{*}{General Advice} & \multirow{1}{*}{Reflection} & \multirow{1}{*}{Total} \\ \hline


501 & 203 & 1172 & 1876 \\ 
\hline

\end{tabular}
\vspace{0mm}
\caption{Results dataset with expert-crafted dialogue scripts.}
% \label{tab:dialogue_overview}
\vspace{-4mm}
\end{table}

==> tables/study_2_test.tex <==
\begin{table*}[!htbp]
\centering
\renewcommand{\arraystretch}{1.0}
% \small
\scriptsize
\setlength{\tabcolsep}{2pt} % Reduce column separation
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}p{3.2cm}p{3.2cm}p{3.2cm}p{2.0cm}p{2.0cm}@{}}
\hline

\multirow{1}{*}{\textbf{Measures}} & \multirow{1}{*}{\textbf{Conditions}} & \textbf{Mean} & \textbf{Effect Size ($r$)} & \textbf{p-value} \\ \hline

Linguistic Quality
 & LLM-SAG vs. LLM-SSAG & 3.95 (0.23) vs. 3.60 (0.18) & 0.43 (large) & 0.01 $**$ \\ 

Dialogue Relevance
 & LLM-SAG vs. LLM-SSAG & 3.39 (0.68) vs. 3.38 (0.51) & 0.09 (small) & 0.54 \\ 
 
Empathy
 & LLM-SAG vs. LLM-SSAG & 3.07 (0.16) vs. 2.94 (0.15) & 0.07 (small) & 0.67 \\ 

Engagement
 & LLM-SAG vs. LLM-SSAG & 2.90 (0.33) vs. 2.58 (0.54) & 0.36 (medium) & 0.02 $*$ \\ 

Perceived MI Level
 & LLM-SAG vs. LLM-SSAG & 3.74 (0.13) vs. 3.31 (0.12) & 0.40 (medium) & 0.01 $**$\\ 

Motivation Change
 & LLM-SAG vs. LLM-SSAG & 3.42 (0.00) vs. 3.00 (0.00) & 0.35 (medium) & 0.02 $*$ \\ 
 
Therapeutic Alliance
 & LLM-SAG vs. LLM-SSAG & 3.58 (0.46) vs. 3.33 (0.48) & 0.27 (medium) & 0.08 \\ 

Usability
 & LLM-SAG vs. LLM-SSAG & 3.82 (0.26) vs. 3.61 (0.26) & 0.24 (medium) & 0.11 \\ 
\hline 

\end{tabular*}
\vspace{-0mm}
\caption{Results from Wilcoxon signed-rank test~\cite{wilcon} for pairwisely comparing the LLM-powered chatbots aligned with expert-crafted dialogue scripts through either prompting (LLM-SAG) or fine-tuning (LLM-SSAG). (**$p$<.01, *$p$<.05)}
\label{tab:analysis_results_2}
\vspace{-0mm}
\end{table*}
